Combining Multiple Cues for Visual Madlibs Question Answering

This paper presents an approach for answering fill-in-the-blank multiple choice questions from the Visual Madlibs dataset. Instead of generic and commonly used representations trained on the ImageNet classification task, our approach employs a combination of networks trained for specialized tasks such as scene recognition, person activity classification, and attribute prediction. We also present a method for localizing phrases from candidate answers in order to provide spatial support for feature extraction. We map each of these features, together with candidate answers, to a joint embedding space through normalized canonical correlation analysis (nCCA). Finally, we solve an optimization problem to learn to combine scores from nCCA models trained on multiple cues to select the best answer. Extensive experimental results show a significant improvement over the previous state of the art and confirm that answering questions from a wide range of types benefits from examining a variety of image cues and carefully choosing the spatial support for feature extraction.

==> cross_expts.tex <==
In Table~\ref{table:madlibs_cross_accuracy}, we explore whether an embedding space learned on a particular question type can be transferred to another question type. We train an nCCA model to learn an embedding space to answer the question type shown in the rows of Table~\ref{table:madlibs_cross_accuracy}, and evaluate that embedding for related question types. For example, in the first row, the embedding from an nCCA trained on Type 1) Scene questions, is evaluated on itself, Type 8) Person Location, and Type 12) Object Location. In almost all cases, the best performance is obtained when the training and testing question types are the same, which is unsurprising. It is surprising that the embedding space learned for answering Type 8) Person Location gives better performance on Type 1) Scene questions than the model trained on Type 1) Scene questions. Further, we do observe that embeddings transfer well for related question types, \eg a model trained on Type 4) Past performs just 0.7\% worse on Type 5) Future, than a model trained on Type 5) Future. To summarize, related question types that rely on similar input cues allow good model transfer. The observed transfer results lead us to the question of whether we can train a single model for multiple question types, which are related. Sharing would increase the amount of training data available for the model being trained, and might also help regularize the embedding space learned, and is explored in the following section~\ref{sec:shared}

\begin{table*}[tb!]
	\setlength{\tabcolsep}{1pt}
	\footnotesize
	\begin{center}
    \resizebox{\textwidth}{!}{%
		\begin{tabular}{l|cl|c|c|c|c|c|c|c|c|c|c|c|c|c} 
            \cline{5-16}
             \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{12}{c}{\bf Tested On} \\\hline
             \multirow{3}{*}{Type} & & \multirow{3}{*}{\bf Trained On} & \multirow{3}{*}{Used Feature} & \multicolumn{5}{c|}{(A)} & \multicolumn{4}{c|}{(B)} & \multicolumn{3}{c}{(C)}\\
             & & & & \multicolumn{1}{c}{1)} & \multicolumn{1}{c}{2)} & \multicolumn{1}{c}{3)} & \multicolumn{1}{c}{4)} & \multicolumn{1}{c|}{5)} & \multicolumn{1}{c}{6)}  & \multicolumn{1}{c}{7)} & \multicolumn{1}{c}{8)} & \multicolumn{1}{c|}{9)} & \multicolumn{1}{c}{10)} & \multicolumn{1}{c}{11)} & \multicolumn{1}{c}{12)} \\
              & & &  & Scene & Emotion & Interesting & Past & Future & Per. Attr. & Per. Act.	& Per. Loc. & Per-Obj Rel. & Obj. Attr. & Obj. Aff. & Obj. Loc. \\\hline
            \multirow{14}{*}{easy} & \multirow{5}{*}{(A)} & 1) Scene & Places & \cellcolor{green!50}{89.04} & & & & & & & 83.68 & & & & 52.39 \\
            & & 2) Emotion & Places & & \cellcolor{green!50}{\bf 49.53} & & & & & & & & & & \\
            & & 3) Interesting & HICO+MPII+Attr. & & & \cellcolor{green!50}{\bf 79.94} & 77.67 & 77.39 & 51.30 & 51.30 & & & & & \\
            & & 4) Past & HICO+MPII+Attr. & & & 79.23 & \cellcolor{green!50}{\bf 84.09} & 82.78 & & 82.16 & & 56.98 & & & \\
            & & 5) Future & HICO+MPII+Attr. & & & 78.19 & 83.38 & \cellcolor{green!50}{\bf 84.97} & 50.37 & 81.94 & & 54.29 & & \\\cline{2-16}
            & \multirow{6}{*}{(B)} & 6) Per. Attr. & HICO+MPII+Attr. & & & & & & \cellcolor{green!50}{\bf 68.43} & 71.67 & & & & & \\
            & & 7) Per. Act. & HICO+MPII+Attr. & & & & & & 39.80 & \cellcolor{green!50}{\bf 87.26} & & 66.31 & & & \\
            & & 8) Per. Loc. & Places & \cellcolor{red!50}{\bf 90.41} & & & & & & & \cellcolor{green!50}{\bf 85.70} & 51.32 & & & 56.61 \\\cline{3-16}
            & & 9) Per-Obj Rel. & HICO+MPII+Attr. & & & & & & & 82.30 & & \cellcolor{green!50}{75.66} & & & \\
            & & 9) Per-Obj Rel. & HICO  & & & & & & & 81.89 & & \cellcolor{green!50}{\bf 75.77} & & & \\
            & & 9) Per-Obj Rel. & Obj. Box ImageNet & & & & & & & & & \cellcolor{green!50}{74.39} & & 73.81 & \\\cline{2-16}
            & \multirow{3}{*}{(C)} & 10) Obj. Attr. & & & & & & & & & & & & \\
            & & 11) Obj. Aff. & Obj. Box ImageNet & & & & & & & & & 62.57 & & \cellcolor{green!50}{\bf 87.20} & \\
            & & 12) Obj. Loc. & Places & 82.76 & & & & & & & 79.92 & & & & \cellcolor{green!50}{\bf 69.41} \\
            \hline\hline
            %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
            \multirow{14}{*}{hard} & \multirow{5}{*}{(A)} & 1) Scene & Places & \cellcolor{green!50}{\bf 73.22} & & & & & & & 63.16 & & & & 38.35 \\
            & & 2) Emotion & Places & & \cellcolor{green!50}{\bf 35.77} & & & & & & & & & & \\
            & & 3) Interesting & HICO+MPII+Attr. & & & \cellcolor{green!50}{\bf 55.37} & 52.68 & 52.38 &  &  & & & & & \\
            & & 4) Past & HICO+MPII+Attr. & & & 54.50 & \cellcolor{green!50}{\bf 58.17} & 56.46 & & 64.08 & & 40.34 & & & \\
            & & 5) Future & HICO+MPII+Attr. & & & 54.23 & 57.03 & \cellcolor{green!50}{\bf 59.98} & 40.31 & 64.35 & & 38.79 & & \\\cline{2-16}
            & \multirow{6}{*}{(B)} & 6) Per. Attr. & HICO+MPII+Attr. & & & & & & \cellcolor{green!50}{\bf 56.17} & 57.91 & & & & & \\
            & & 7) Per. Act. & HICO+MPII+Attr. & & & & & & 30.19 & \cellcolor{green!50}{\bf 71.42} & & 48.36 & & & \\
            & & 8) Per. Loc. & Places & 72.71 & & & & & & & \cellcolor{green!50}{\bf 66.66} & 36.50 & & & 43.03 \\\cline{3-16}
            & & 9) Per-Obj Rel. & HICO+MPII+Attr. & & & & & & & 65.37 & & \cellcolor{green!50}{56.88} & & & \\
            & & 9) Per-Obj Rel. & HICO  & & & & & & & 66.97 & & \cellcolor{green!50}{\bf 58.72} & & & \\
            & & 9) Per-Obj Rel. & Obj. Box ImageNet & & & & & & & & & \cellcolor{green!50}{55.85} & & 48.39 & \\\cline{2-16}
            & \multirow{3}{*}{(C)} & 10) Obj. Attr. & & & & & & & & & & & & \\
            & & 11) Obj. Aff. & Obj. Box ImageNet & & & & & & & & & 42.17 & & \cellcolor{green!50}{\bf 67.65} & \\
            & & 12) Obj. Loc. & Places & 59.71 & & & & & & & 55.46 & & & & \cellcolor{green!50}{\bf 57.34} \\
            \hline
        \end{tabular}
        }\vspace{-2mm}
	\end{center}
\caption{Accuracy on Madlibs questions when CCA embeddings trained on the question type in the rows are tested on question types in the columns. This measures if embeddings spaces for one question type are useful for another question type. Green cells indicate cases where training and testing sets are the same. Bold values indicate maximum accuracy per column}
	\label{table:madlibs_cross_accuracy}
    %\vspace{-4mm}
\end{table*}
